Inference for Linear Conditional Moment Inequalities

We show that moment inequalities in a wide variety of economic applications have a particular linear conditional structure. We use this structure to construct uniformly valid confidence sets that remain computationally tractable even in settings with nuisance parameters. We first introduce least favorable critical values which deliver non-conservative tests if all moments are binding. Next, we introduce a novel conditional inference approach which ensures a strong form of insensitivity to slack moments. Our recommended approach is a hybrid technique which combines desirable aspects of the least favorable and conditional methods. The hybrid approach performs well in simulations calibrated to Wollmann (2018), with favorable power and computational time comparisons relative to existing alternatives.

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table05.tex <==
$2$ & $6$ & $2.06$ & $2.13$ & $1.81$ & $3.39$ \\ 
$2$ & $14$ & $5.26$ & $4.79$ & $3.16$ & $7.42$ \\ 
$4$ & $14$ & $3.88$ & $2.42$ & $2.42$ & $5.52$ \\ 
$4$ & $38$ & $11.48$ & $7.50$ & $3.76$ & $14.83$ \\ 
$10$ & $38$ & $7.82$ & $2.44$ & $2.44$ & $10.35$ \\ 
$10$ & $110$ & $18.78$ & $11.67$ & $7.24$ & $22.34$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table05_asandkms.tex <==
$2.04$ & $1.98$ \\ 
$4.38$ & $4.36$ \\ 
$2.07$ & $1.06$ \\ 
$10.79$ & $10.08$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table05_coxandshi.tex <==
$2$ & $6$ & $2.06$ & $2.13$ & $1.81$ & $3.39$ & $2.78$ & $2.13$ \\ 
$2$ & $14$ & $5.26$ & $4.79$ & $3.16$ & $7.42$ & $4.46$ & $3.16$ \\ 
$4$ & $14$ & $3.88$ & $2.42$ & $2.42$ & $5.52$ & $2.75$ & $2.42$ \\ 
$4$ & $38$ & $11.48$ & $7.50$ & $3.76$ & $14.83$ & $5.39$ & $4.10$ \\ 
$10$ & $38$ & $7.82$ & $2.44$ & $2.44$ & $10.35$ & $3.09$ & $2.44$ \\ 
$10$ & $110$ & $18.78$ & $11.67$ & $7.24$ & $22.34$ & $13.90$ & $13.90$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table05_zerocutoff.tex <==
$2$ & $6$ & $2.12$ & $2.19$ & $1.86$ & $3.45$ \\ 
$2$ & $14$ & $6.26$ & $5.79$ & $4.16$ & $8.42$ \\ 
$4$ & $14$ & $3.94$ & $2.48$ & $2.48$ & $5.58$ \\ 
$4$ & $38$ & $12.51$ & $8.54$ & $4.80$ & $15.87$ \\ 
$10$ & $38$ & $7.89$ & $2.51$ & $2.51$ & $10.42$ \\ 
$10$ & $110$ & $21.62$ & $14.52$ & $10.08$ & $25.18$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table05_zerocutoff_asandkms.tex <==
$2.10$ & $2.04$ \\ 
$5.38$ & $5.36$ \\ 
$2.12$ & $1.12$ \\ 
$11.82$ & $11.12$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table05_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $2.12$ & $2.19$ & $1.86$ & $3.45$ & $2.84$ & $2.19$ \\ 
$2$ & $14$ & $6.26$ & $5.79$ & $4.16$ & $8.42$ & $5.46$ & $4.16$ \\ 
$4$ & $14$ & $3.94$ & $2.48$ & $2.48$ & $5.58$ & $2.81$ & $2.48$ \\ 
$4$ & $38$ & $12.51$ & $8.54$ & $4.80$ & $15.87$ & $6.43$ & $5.14$ \\ 
$10$ & $38$ & $7.89$ & $2.51$ & $2.51$ & $10.42$ & $3.16$ & $2.51$ \\ 
$10$ & $110$ & $21.62$ & $14.52$ & $10.08$ & $25.18$ & $16.74$ & $16.74$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50.tex <==
$2$ & $6$ & $3.99$ & $4.08$ & $3.76$ & $5.33$ \\ 
$2$ & $14$ & $10.30$ & $10.31$ & $8.36$ & $12.57$ \\ 
$4$ & $14$ & $5.92$ & $4.37$ & $4.37$ & $7.57$ \\ 
$4$ & $38$ & $16.14$ & $14.49$ & $11.56$ & $18.88$ \\ 
$10$ & $38$ & $10.21$ & $4.72$ & $4.72$ & $12.71$ \\ 
$10$ & $110$ & $22.24$ & $17.80$ & $14.25$ & $25.50$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_allcombined_modified.tex <==
$2$ & $6$ & $3.99$ & $4.08$ & $3.76$ & $5.33$ & $4.73$ & $4.08$ & $4.32$ & $4.14$ \\ 
$2$ & $14$ & $10.30$ & $10.31$ & $8.36$ & $12.57$ & $9.66$ & $8.36$ & $9.99$ & $9.80$ \\ 
$4$ & $14$ & $5.92$ & $4.37$ & $4.37$ & $7.57$ & $5.02$ & $4.37$ & $5.93$ & $5.38$ \\ 
$4$ & $38$ & $16.14$ & $14.49$ & $11.56$ & $18.88$ & $12.86$ & $12.54$ & $16.08$ & $15.41$ \\ 
$10$ & $38$ & $10.21$ & $4.72$ & $4.72$ & $12.71$ & $5.37$ & $4.72$ & $ $ & $ $ \\ 
$10$ & $110$ & $22.24$ & $17.80$ & $14.25$ & $25.50$ & $18.45$ & $18.45$ & $ $ & $ $\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_asandkms.tex <==
$2$ & $6$ & $3.99$ & $4.08$ & $3.76$ & $5.33$ & $4.12$ & $4.14$ \\ 
$2$ & $14$ & $10.30$ & $10.31$ & $8.36$ & $12.57$ & $9.67$ & $9.80$ \\ 
$4$ & $14$ & $5.92$ & $4.37$ & $4.37$ & $7.57$ & $5.82$ & $5.38$ \\ 
$4$ & $38$ & $16.14$ & $14.49$ & $11.56$ & $18.88$ & $15.90$ & $15.41$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_asandkms_only.tex <==
$4.12$ & $4.14$ \\ 
$9.67$ & $9.80$ \\ 
$5.82$ & $5.38$ \\ 
$15.90$ & $15.41$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_coxandshi.tex <==
$2$ & $6$ & $3.99$ & $4.08$ & $3.76$ & $5.33$ & $4.73$ & $4.08$ \\ 
$2$ & $14$ & $10.30$ & $10.31$ & $8.36$ & $12.57$ & $9.66$ & $8.36$ \\ 
$4$ & $14$ & $5.92$ & $4.37$ & $4.37$ & $7.57$ & $5.02$ & $4.37$ \\ 
$4$ & $38$ & $16.14$ & $14.49$ & $11.56$ & $18.88$ & $12.86$ & $12.54$ \\ 
$10$ & $38$ & $10.21$ & $4.72$ & $4.72$ & $12.71$ & $5.37$ & $4.72$ \\ 
$10$ & $110$ & $22.24$ & $17.80$ & $14.25$ & $25.50$ & $18.45$ & $18.45$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_zerocutoff.tex <==
$2$ & $6$ & $4.05$ & $4.14$ & $3.81$ & $5.38$ \\ 
$2$ & $14$ & $11.30$ & $11.31$ & $9.36$ & $13.57$ \\ 
$4$ & $14$ & $5.98$ & $4.43$ & $4.43$ & $7.63$ \\ 
$4$ & $38$ & $17.18$ & $15.53$ & $12.60$ & $19.92$ \\ 
$10$ & $38$ & $10.28$ & $4.79$ & $4.79$ & $12.78$ \\ 
$10$ & $110$ & $25.08$ & $20.64$ & $17.10$ & $28.34$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_zerocutoff_allcombined.tex <==
$2$ & $6$ & $4.05$ & $4.14$ & $3.81$ & $5.38$ & $4.79$ & $4.14$ & $4.18$ & $4.20$ \\ 
$2$ & $14$ & $11.30$ & $11.31$ & $9.36$ & $13.57$ & $10.66$ & $9.36$ & $10.67$ & $10.81$ \\ 
$4$ & $14$ & $5.98$ & $4.43$ & $4.43$ & $7.63$ & $5.08$ & $4.43$ & $5.87$ & $5.44$ \\ 
$4$ & $38$ & $17.18$ & $15.53$ & $12.60$ & $19.92$ & $13.90$ & $13.58$ & $16.94$ & $16.45$ \\ 
$10$ & $38$ & $10.28$ & $4.79$ & $4.79$ & $12.78$ & $5.44$ & $4.79$ & $ $ & $ $ \\ 
$10$ & $110$ & $25.08$ & $20.64$ & $17.10$ & $28.34$ & $21.29$ & $21.29$ & $ $ & $ $\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_zerocutoff_asandkms.tex <==
$2$ & $6$ & $4.05$ & $4.14$ & $3.81$ & $5.38$ & $4.18$ & $4.20$ \\ 
$2$ & $14$ & $11.30$ & $11.31$ & $9.36$ & $13.57$ & $10.67$ & $10.81$ \\ 
$4$ & $14$ & $5.98$ & $4.43$ & $4.43$ & $7.63$ & $5.87$ & $5.44$ \\ 
$4$ & $38$ & $17.18$ & $15.53$ & $12.60$ & $19.92$ & $16.94$ & $16.45$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_zerocutoff_asandkms_only.tex <==
$4.18$ & $4.20$ \\ 
$10.67$ & $10.81$ \\ 
$5.87$ & $5.44$ \\ 
$16.94$ & $16.45$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table50_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $4.05$ & $4.14$ & $3.81$ & $5.38$ & $4.79$ & $4.14$ \\ 
$2$ & $14$ & $11.30$ & $11.31$ & $9.36$ & $13.57$ & $10.66$ & $9.36$ \\ 
$4$ & $14$ & $5.98$ & $4.43$ & $4.43$ & $7.63$ & $5.08$ & $4.43$ \\ 
$4$ & $38$ & $17.18$ & $15.53$ & $12.60$ & $19.92$ & $13.90$ & $13.58$ \\ 
$10$ & $38$ & $10.28$ & $4.79$ & $4.79$ & $12.78$ & $5.44$ & $4.79$ \\ 
$10$ & $110$ & $25.08$ & $20.64$ & $17.10$ & $28.34$ & $21.29$ & $21.29$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table95.tex <==
$2$ & $6$ & $6.17$ & $6.19$ & $6.03$ & $7.45$ \\ 
$2$ & $14$ & $15.81$ & $18.11$ & $15.84$ & $17.81$ \\ 
$4$ & $14$ & $8.08$ & $6.48$ & $6.65$ & $9.79$ \\ 
$4$ & $38$ & $19.58$ & $20.01$ & $17.41$ & $21.87$ \\ 
$10$ & $38$ & $12.64$ & $7.32$ & $7.32$ & $15.22$ \\ 
$10$ & $110$ & $25.47$ & $23.32$ & $19.75$ & $28.32$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table95_asandkms.tex <==
$6.28$ & $6.48$ \\ 
$15.62$ & $15.72$ \\ 
$8.29$ & $7.60$ \\ 
$19.36$ & $19.11$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table95_coxandshi.tex <==
$2$ & $6$ & $6.17$ & $6.19$ & $6.03$ & $7.45$ & $6.68$ & $6.19$ \\ 
$2$ & $14$ & $15.81$ & $18.11$ & $15.84$ & $17.81$ & $15.51$ & $14.86$ \\ 
$4$ & $14$ & $8.08$ & $6.48$ & $6.65$ & $9.79$ & $7.13$ & $6.48$ \\ 
$4$ & $38$ & $19.58$ & $20.01$ & $17.41$ & $21.87$ & $17.41$ & $17.09$ \\ 
$10$ & $38$ & $12.64$ & $7.32$ & $7.32$ & $15.22$ & $7.64$ & $7.32$ \\ 
$10$ & $110$ & $25.47$ & $23.32$ & $19.75$ & $28.32$ & $22.67$ & $22.67$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table95_zerocutoff.tex <==
$2$ & $6$ & $6.23$ & $6.25$ & $6.09$ & $7.51$ \\ 
$2$ & $14$ & $16.81$ & $19.11$ & $16.84$ & $18.81$ \\ 
$4$ & $14$ & $8.14$ & $6.54$ & $6.71$ & $9.85$ \\ 
$4$ & $38$ & $20.61$ & $21.05$ & $18.45$ & $22.91$ \\ 
$10$ & $38$ & $12.71$ & $7.39$ & $7.39$ & $15.29$ \\ 
$10$ & $110$ & $28.31$ & $26.16$ & $22.59$ & $31.16$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table95_zerocutoff_asandkms.tex <==
$6.34$ & $6.54$ \\ 
$16.62$ & $16.72$ \\ 
$8.35$ & $7.65$ \\ 
$20.40$ & $20.14$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_table95_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $6.23$ & $6.25$ & $6.09$ & $7.51$ & $6.74$ & $6.25$ \\ 
$2$ & $14$ & $16.81$ & $19.11$ & $16.84$ & $18.81$ & $16.51$ & $15.86$ \\ 
$4$ & $14$ & $8.14$ & $6.54$ & $6.71$ & $9.85$ & $7.19$ & $6.54$ \\ 
$4$ & $38$ & $20.61$ & $21.05$ & $18.45$ & $22.91$ & $18.45$ & $18.13$ \\ 
$10$ & $38$ & $12.71$ & $7.39$ & $7.39$ & $15.29$ & $7.71$ & $7.39$ \\ 
$10$ & $110$ & $28.31$ & $26.16$ & $22.59$ & $31.16$ & $25.51$ & $25.51$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_tablemean.tex <==
$2$ & $6$ & $4.05$ & $4.08$ & $3.93$ & $5.38$ \\ 
$2$ & $14$ & $10.43$ & $10.71$ & $8.59$ & $12.61$ \\ 
$4$ & $14$ & $5.95$ & $4.29$ & $4.31$ & $7.60$ \\ 
$4$ & $38$ & $15.83$ & $14.24$ & $11.05$ & $18.60$ \\ 
$10$ & $38$ & $10.24$ & $4.94$ & $4.86$ & $12.77$ \\ 
$10$ & $110$ & $22.16$ & $17.79$ & $14.06$ & $25.43$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_tablemean_asandkms.tex <==
$ $ & $ $ \\ 
$ $ & $ $ \\ 
$ $ & $ $ \\ 
$ $ & $ $\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_tablemean_coxandshi.tex <==
$2$ & $6$ & $4.05$ & $4.08$ & $3.93$ & $5.38$ & $4.67$ & $4.08$ \\ 
$2$ & $14$ & $10.43$ & $10.71$ & $8.59$ & $12.61$ & $9.73$ & $8.53$ \\ 
$4$ & $14$ & $5.95$ & $4.29$ & $4.31$ & $7.60$ & $4.90$ & $4.29$ \\ 
$4$ & $38$ & $15.83$ & $14.24$ & $11.05$ & $18.60$ & $12.29$ & $11.82$ \\ 
$10$ & $38$ & $10.24$ & $4.94$ & $4.86$ & $12.77$ & $5.45$ & $4.77$ \\ 
$10$ & $110$ & $22.16$ & $17.79$ & $14.06$ & $25.43$ & $18.39$ & $18.39$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_tablemean_zerocutoff.tex <==
$2$ & $6$ & $4.11$ & $4.14$ & $3.99$ & $5.44$ \\ 
$2$ & $14$ & $11.43$ & $11.71$ & $9.60$ & $13.61$ \\ 
$4$ & $14$ & $6.01$ & $4.35$ & $4.37$ & $7.65$ \\ 
$4$ & $38$ & $16.87$ & $15.28$ & $12.09$ & $19.63$ \\ 
$10$ & $38$ & $10.31$ & $5.01$ & $4.93$ & $12.84$ \\ 
$10$ & $110$ & $25$ & $20.63$ & $16.90$ & $28.27$\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_tablemean_zerocutoff_asandkms.tex <==
$ $ & $ $ \\ 
$ $ & $ $ \\ 
$ $ & $ $ \\ 
$ $ & $ $\\

==> Tables/Mean_Weight_Rejection_Probabilities_excess_length_tablemean_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $4.11$ & $4.14$ & $3.99$ & $5.44$ & $4.73$ & $4.14$ \\ 
$2$ & $14$ & $11.43$ & $11.71$ & $9.60$ & $13.61$ & $10.74$ & $9.53$ \\ 
$4$ & $14$ & $6.01$ & $4.35$ & $4.37$ & $7.65$ & $4.96$ & $4.35$ \\ 
$4$ & $38$ & $16.87$ & $15.28$ & $12.09$ & $19.63$ & $13.33$ & $12.86$ \\ 
$10$ & $38$ & $10.31$ & $5.01$ & $4.93$ & $12.84$ & $5.52$ & $4.84$ \\ 
$10$ & $110$ & $25$ & $20.63$ & $16.90$ & $28.27$ & $21.23$ & $21.23$\\

==> Tables/Mean_Weight_Rejection_Probabilities_lower_bound_sizes.tex <==
$2$ & $6$ & $0.02$ & $0.02$ & $0.02$ & $0.00$ \\ 
$2$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$4$ & $14$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.02$ & $0.01$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.01$ & $0.01$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_lower_bound_sizes_zerocutoff.tex <==
$2$ & $6$ & $0.02$ & $0.02$ & $0.02$ & $0.00$ \\ 
$2$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$4$ & $14$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.01$ & $0.00$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.01$ & $0.01$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ \\ 
$0.00$ & $0.02$ & $0.01$ & $0.00$ \\ 
$0.00$ & $0.07$ & $0.07$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_allcombined_modified.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ & $0.02$ & $0.05$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ & $0.01$ & $0.03$ & $0.00$ & $0.00$ \\ 
$0.00$ & $0.02$ & $0.01$ & $0.00$ & $0.01$ & $0.02$ & $ $ & $ $ \\ 
$0.00$ & $0.07$ & $0.07$ & $0.00$ & $0.00$ & $0.00$ & $ $ & $ $\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_asandkms.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ & $0.02$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.02$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.03$ & $0.05$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ & $0.00$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_coxandshi.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ & $0.01$ & $0.03$ \\ 
$0.00$ & $0.02$ & $0.01$ & $0.00$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.07$ & $0.07$ & $0.00$ & $0.00$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_zerocutoff.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$0.00$ & $0.03$ & $0.02$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_zerocutoff_allcombined.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ & $0.02$ & $0.02$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.01$ & $0.01$ & $0.02$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ & $0.03$ & $0.05$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.00$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.01$ & $0.01$ & $ $ & $ $ \\ 
$0.00$ & $0.03$ & $0.02$ & $0.00$ & $0.00$ & $0.00$ & $ $ & $ $\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_zerocutoff_asandkms.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ & $0.02$ & $0.02$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.02$ & $0.02$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.03$ & $0.05$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.00$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_max_size_in_id_set_zerocutoff_coxandshi.tex <==
$0.02$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.01$ & $0.01$ \\ 
$0.00$ & $0.02$ & $0.02$ & $0.00$ & $0.01$ & $0.02$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.01$ & $0.01$ \\ 
$0.00$ & $0.01$ & $0.01$ & $0.00$ & $0.01$ & $0.01$ \\ 
$0.00$ & $0.03$ & $0.02$ & $0.00$ & $0.00$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_power_table05.tex <==
$2$ & $6$ & $3.04$ & $2.74$ & $2.74$ & $2.77$ & $2.23$ & $83.46$ & $84.04$ & $84.07$ & $83.95$ & $84.86$ \\ 
$2$ & $14$ & $26.10$ & $24.77$ & $25.36$ & $25.36$ & $24.16$ & $72.99$ & $75.18$ & $73.71$ & $73.71$ & $76.76$ \\ 
$4$ & $14$ & $3.27$ & $2.43$ & $2.92$ & $2.92$ & $1.93$ & $83.40$ & $85.30$ & $84.18$ & $84.22$ & $86.41$ \\ 
$4$ & $38$ & $26.40$ & $23.99$ & $25.59$ & $25.55$ & $23.20$ & $73.01$ & $80.22$ & $73.76$ & $73.93$ & $82.70$ \\ 
$10$ & $38$ & $5.83$ & $3.94$ & $5.43$ & $5.39$ & $3.20$ & $82.04$ & $86.97$ & $83.03$ & $83.04$ & $88.71$ \\ 
$10$ & $110$ & $29.20$ & $24.01$ & $28.02$ & $27.99$ & $22.93$ & $73.15$ & $84.95$ & $71.65$ & $72.08$ & $87.60$\\

==> Tables/Mean_Weight_Rejection_Probabilities_power_table50.tex <==
$2$ & $6$ & $3.04$ & $1.55$ & $1.54$ & $1.60$ & $1.04$ & $83.46$ & $86.01$ & $86.05$ & $85.95$ & $86.86$ \\ 
$2$ & $14$ & $26.10$ & $22.85$ & $23.42$ & $23.42$ & $22.24$ & $72.99$ & $80.26$ & $78.72$ & $78.73$ & $81.91$ \\ 
$4$ & $14$ & $3.27$ & $1.27$ & $1.75$ & $1.75$ & $0.72$ & $83.40$ & $87.34$ & $86.15$ & $86.17$ & $88.44$ \\ 
$4$ & $38$ & $26.40$ & $22.04$ & $23.62$ & $23.56$ & $21.23$ & $73.01$ & $84.68$ & $81.21$ & $81.28$ & $86.62$ \\ 
$10$ & $38$ & $5.83$ & $2.72$ & $4.23$ & $4.21$ & $1.97$ & $82.04$ & $89.20$ & $85.20$ & $85.26$ & $90.96$ \\ 
$10$ & $110$ & $29.20$ & $21.95$ & $25.87$ & $25.79$ & $20.84$ & $73.15$ & $88.22$ & $86.19$ & $85.87$ & $90.33$\\

==> Tables/Mean_Weight_Rejection_Probabilities_power_table95.tex <==
$2$ & $6$ & $3.04$ & $0.30$ & $0.29$ & $0.37$ & $-0.18$ & $83.46$ & $88$ & $88.02$ & $87.94$ & $88.85$ \\ 
$2$ & $14$ & $26.10$ & $20.99$ & $21.60$ & $21.57$ & $20.36$ & $72.99$ & $85.08$ & $97.87$ & $85.56$ & $86.52$ \\ 
$4$ & $14$ & $3.27$ & $0.05$ & $0.51$ & $0.52$ & $-0.52$ & $83.40$ & $89.41$ & $88.21$ & $88.29$ & $90.54$ \\ 
$4$ & $38$ & $26.40$ & $20.18$ & $21.78$ & $21.69$ & $19.36$ & $73.01$ & $88.08$ & $97.49$ & $88.06$ & $89.41$ \\ 
$10$ & $38$ & $5.83$ & $1.49$ & $3.03$ & $2.98$ & $0.74$ & $82.04$ & $91.53$ & $87.52$ & $87.51$ & $93.32$ \\ 
$10$ & $110$ & $29.20$ & $19.99$ & $23.22$ & $23.22$ & $18.83$ & $73.15$ & $90.93$ & $102.95$ & $90.30$ & $92.86$\\

==> Tables/Mean_Weight_Rejection_Probabilities_upper_bound_sizes.tex <==
$2$ & $6$ & $0.01$ & $0.01$ & $0.01$ & $0.00$ \\ 
$2$ & $14$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$4$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.04$ & $0.04$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.07$ & $0.07$ & $0.00$\\

==> Tables/Mean_Weight_Rejection_Probabilities_upper_bound_sizes_zerocutoff.tex <==
$2$ & $6$ & $0.01$ & $0.01$ & $0.01$ & $0.00$ \\ 
$2$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$4$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.01$ & $0.00$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.03$ & $0.02$ & $0.00$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table05.tex <==
$2$ & $6$ & $1.06$ & $0.99$ & $0.70$ & $2.72$ \\ 
$2$ & $14$ & $2.06$ & $0.99$ & $0.79$ & $3.55$ \\ 
$4$ & $14$ & $1.82$ & $0.93$ & $0.68$ & $3.61$ \\ 
$4$ & $38$ & $3.37$ & $1.18$ & $1.18$ & $4.58$ \\ 
$10$ & $38$ & $3.22$ & $1.18$ & $1.18$ & $4.72$ \\ 
$10$ & $110$ & $4.13$ & $1.68$ & $1.65$ & $5.55$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table05_asandkms.tex <==
$1.65$ & $1.47$ \\ 
$1.90$ & $1.85$ \\ 
$1.64$ & $1.44$ \\ 
$1.69$ & $0.32$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table05_coxandshi.tex <==
$2$ & $6$ & $1.06$ & $0.99$ & $0.70$ & $2.72$ & $1.74$ & $0.99$ \\ 
$2$ & $14$ & $2.06$ & $0.99$ & $0.79$ & $3.55$ & $1.83$ & $0.99$ \\ 
$4$ & $14$ & $1.82$ & $0.93$ & $0.68$ & $3.61$ & $1.77$ & $0.93$ \\ 
$4$ & $38$ & $3.37$ & $1.18$ & $1.18$ & $4.58$ & $1.93$ & $1.18$ \\ 
$10$ & $38$ & $3.22$ & $1.18$ & $1.18$ & $4.72$ & $2.05$ & $1.18$ \\ 
$10$ & $110$ & $4.13$ & $1.68$ & $1.65$ & $5.55$ & $3.43$ & $2.68$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table05_zerocutoff.tex <==
$2$ & $6$ & $1.14$ & $1.07$ & $0.78$ & $2.80$ \\ 
$2$ & $14$ & $2.14$ & $1.07$ & $0.88$ & $3.63$ \\ 
$4$ & $14$ & $1.91$ & $1.02$ & $0.76$ & $3.70$ \\ 
$4$ & $38$ & $3.46$ & $1.26$ & $1.26$ & $4.66$ \\ 
$10$ & $38$ & $3.30$ & $1.26$ & $1.26$ & $4.81$ \\ 
$10$ & $110$ & $4.21$ & $1.76$ & $1.73$ & $5.64$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table05_zerocutoff_asandkms.tex <==
$1.73$ & $1.55$ \\ 
$1.99$ & $1.93$ \\ 
$1.73$ & $1.52$ \\ 
$1.77$ & $0.40$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table05_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $1.14$ & $1.07$ & $0.78$ & $2.80$ & $1.82$ & $1.07$ \\ 
$2$ & $14$ & $2.14$ & $1.07$ & $0.88$ & $3.63$ & $1.91$ & $1.07$ \\ 
$4$ & $14$ & $1.91$ & $1.02$ & $0.76$ & $3.70$ & $1.86$ & $1.02$ \\ 
$4$ & $38$ & $3.46$ & $1.26$ & $1.26$ & $4.66$ & $2.01$ & $1.26$ \\ 
$10$ & $38$ & $3.30$ & $1.26$ & $1.26$ & $4.81$ & $2.14$ & $1.26$ \\ 
$10$ & $110$ & $4.21$ & $1.76$ & $1.73$ & $5.64$ & $3.51$ & $2.76$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50.tex <==
$2$ & $6$ & $4.29$ & $4.20$ & $3.95$ & $6.04$ \\ 
$2$ & $14$ & $5.41$ & $4.45$ & $4.20$ & $6.93$ \\ 
$4$ & $14$ & $5.19$ & $4.43$ & $4.18$ & $6.99$ \\ 
$4$ & $38$ & $6.68$ & $4.43$ & $4.43$ & $7.97$ \\ 
$10$ & $38$ & $6.58$ & $4.43$ & $4.43$ & $8.09$ \\ 
$10$ & $110$ & $7.69$ & $5.18$ & $5.18$ & $9.11$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_allcombined_modified.tex <==
$2$ & $6$ & $4.29$ & $4.20$ & $3.95$ & $6.04$ & $4.95$ & $4.20$ & $4.94$ & $4.74$ \\ 
$2$ & $14$ & $5.41$ & $4.45$ & $4.20$ & $6.93$ & $5.20$ & $4.45$ & $5.40$ & $5.26$ \\ 
$4$ & $14$ & $5.19$ & $4.43$ & $4.18$ & $6.99$ & $5.18$ & $4.43$ & $5.66$ & $5.13$ \\ 
$4$ & $38$ & $6.68$ & $4.43$ & $4.43$ & $7.97$ & $5.43$ & $4.43$ & $6.43$ & $6.08$ \\ 
$10$ & $38$ & $6.58$ & $4.43$ & $4.43$ & $8.09$ & $5.43$ & $4.43$ & $ $ & $ $ \\ 
$10$ & $110$ & $7.69$ & $5.18$ & $5.18$ & $9.11$ & $7.43$ & $7.18$ & $ $ & $ $\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_asandkms.tex <==
$2$ & $6$ & $4.29$ & $4.20$ & $3.95$ & $6.04$ & $4.94$ & $4.74$ \\ 
$2$ & $14$ & $5.41$ & $4.45$ & $4.20$ & $6.93$ & $5.31$ & $5.26$ \\ 
$4$ & $14$ & $5.19$ & $4.43$ & $4.18$ & $6.99$ & $5.48$ & $5.13$ \\ 
$4$ & $38$ & $6.68$ & $4.43$ & $4.43$ & $7.97$ & $6.23$ & $6.08$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_asandkms_only.tex <==
$4.94$ & $4.74$ \\ 
$5.31$ & $5.26$ \\ 
$5.48$ & $5.13$ \\ 
$6.23$ & $6.08$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_coxandshi.tex <==
$2$ & $6$ & $4.29$ & $4.20$ & $3.95$ & $6.04$ & $4.95$ & $4.20$ \\ 
$2$ & $14$ & $5.41$ & $4.45$ & $4.20$ & $6.93$ & $5.20$ & $4.45$ \\ 
$4$ & $14$ & $5.19$ & $4.43$ & $4.18$ & $6.99$ & $5.18$ & $4.43$ \\ 
$4$ & $38$ & $6.68$ & $4.43$ & $4.43$ & $7.97$ & $5.43$ & $4.43$ \\ 
$10$ & $38$ & $6.58$ & $4.43$ & $4.43$ & $8.09$ & $5.43$ & $4.43$ \\ 
$10$ & $110$ & $7.69$ & $5.18$ & $5.18$ & $9.11$ & $7.43$ & $7.18$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_zerocutoff.tex <==
$2$ & $6$ & $4.38$ & $4.28$ & $4.03$ & $6.12$ \\ 
$2$ & $14$ & $5.50$ & $4.53$ & $4.28$ & $7.01$ \\ 
$4$ & $14$ & $5.27$ & $4.51$ & $4.26$ & $7.08$ \\ 
$4$ & $38$ & $6.76$ & $4.51$ & $4.51$ & $8.05$ \\ 
$10$ & $38$ & $6.66$ & $4.51$ & $4.51$ & $8.18$ \\ 
$10$ & $110$ & $7.77$ & $5.26$ & $5.26$ & $9.19$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_zerocutoff_allcombined.tex <==
$2$ & $6$ & $4.38$ & $4.28$ & $4.03$ & $6.12$ & $5.03$ & $4.28$ & $5.02$ & $4.83$ \\ 
$2$ & $14$ & $5.50$ & $4.53$ & $4.28$ & $7.01$ & $5.28$ & $4.53$ & $5.40$ & $5.34$ \\ 
$4$ & $14$ & $5.27$ & $4.51$ & $4.26$ & $7.08$ & $5.26$ & $4.51$ & $5.56$ & $5.22$ \\ 
$4$ & $38$ & $6.76$ & $4.51$ & $4.51$ & $8.05$ & $5.51$ & $4.51$ & $6.31$ & $6.17$ \\ 
$10$ & $38$ & $6.66$ & $4.51$ & $4.51$ & $8.18$ & $5.51$ & $4.51$ & $ $ & $ $ \\ 
$10$ & $110$ & $7.77$ & $5.26$ & $5.26$ & $9.19$ & $7.51$ & $7.26$ & $ $ & $ $\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_zerocutoff_asandkms.tex <==
$2$ & $6$ & $4.38$ & $4.28$ & $4.03$ & $6.12$ & $5.02$ & $4.83$ \\ 
$2$ & $14$ & $5.50$ & $4.53$ & $4.28$ & $7.01$ & $5.40$ & $5.34$ \\ 
$4$ & $14$ & $5.27$ & $4.51$ & $4.26$ & $7.08$ & $5.56$ & $5.22$ \\ 
$4$ & $38$ & $6.76$ & $4.51$ & $4.51$ & $8.05$ & $6.31$ & $6.17$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_zerocutoff_asandkms_only.tex <==
$5.02$ & $4.83$ \\ 
$5.40$ & $5.34$ \\ 
$5.56$ & $5.22$ \\ 
$6.31$ & $6.17$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table50_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $4.38$ & $4.28$ & $4.03$ & $6.12$ & $5.03$ & $4.28$ \\ 
$2$ & $14$ & $5.50$ & $4.53$ & $4.28$ & $7.01$ & $5.28$ & $4.53$ \\ 
$4$ & $14$ & $5.27$ & $4.51$ & $4.26$ & $7.08$ & $5.26$ & $4.51$ \\ 
$4$ & $38$ & $6.76$ & $4.51$ & $4.51$ & $8.05$ & $5.51$ & $4.51$ \\ 
$10$ & $38$ & $6.66$ & $4.51$ & $4.51$ & $8.18$ & $5.51$ & $4.51$ \\ 
$10$ & $110$ & $7.77$ & $5.26$ & $5.26$ & $9.19$ & $7.51$ & $7.26$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table95.tex <==
$2$ & $6$ & $7.49$ & $7.45$ & $7.08$ & $9.18$ \\ 
$2$ & $14$ & $8.70$ & $7.70$ & $7.45$ & $10.23$ \\ 
$4$ & $14$ & $8.51$ & $7.68$ & $7.43$ & $10.22$ \\ 
$4$ & $38$ & $9.99$ & $7.68$ & $7.68$ & $11.31$ \\ 
$10$ & $38$ & $9.86$ & $7.80$ & $7.80$ & $11.44$ \\ 
$10$ & $110$ & $11.10$ & $8.43$ & $8.43$ & $12.54$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table95_asandkms.tex <==
$8.10$ & $7.88$ \\ 
$8.61$ & $8.44$ \\ 
$8.83$ & $8.65$ \\ 
$9.68$ & $9.51$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table95_coxandshi.tex <==
$2$ & $6$ & $7.49$ & $7.45$ & $7.08$ & $9.18$ & $8.20$ & $7.45$ \\ 
$2$ & $14$ & $8.70$ & $7.70$ & $7.45$ & $10.23$ & $8.45$ & $7.70$ \\ 
$4$ & $14$ & $8.51$ & $7.68$ & $7.43$ & $10.22$ & $8.43$ & $7.68$ \\ 
$4$ & $38$ & $9.99$ & $7.68$ & $7.68$ & $11.31$ & $8.68$ & $7.68$ \\ 
$10$ & $38$ & $9.86$ & $7.80$ & $7.80$ & $11.44$ & $8.68$ & $7.80$ \\ 
$10$ & $110$ & $11.10$ & $8.43$ & $8.43$ & $12.54$ & $11.18$ & $11.18$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table95_zerocutoff.tex <==
$2$ & $6$ & $7.58$ & $7.53$ & $7.16$ & $9.27$ \\ 
$2$ & $14$ & $8.78$ & $7.78$ & $7.53$ & $10.32$ \\ 
$4$ & $14$ & $8.59$ & $7.76$ & $7.51$ & $10.31$ \\ 
$4$ & $38$ & $10.08$ & $7.76$ & $7.76$ & $11.40$ \\ 
$10$ & $38$ & $9.95$ & $7.89$ & $7.89$ & $11.52$ \\ 
$10$ & $110$ & $11.19$ & $8.51$ & $8.51$ & $12.63$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table95_zerocutoff_asandkms.tex <==
$8.18$ & $7.96$ \\ 
$8.69$ & $8.52$ \\ 
$8.92$ & $8.73$ \\ 
$9.77$ & $9.59$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_table95_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $7.58$ & $7.53$ & $7.16$ & $9.27$ & $8.28$ & $7.53$ \\ 
$2$ & $14$ & $8.78$ & $7.78$ & $7.53$ & $10.32$ & $8.53$ & $7.78$ \\ 
$4$ & $14$ & $8.59$ & $7.76$ & $7.51$ & $10.31$ & $8.51$ & $7.76$ \\ 
$4$ & $38$ & $10.08$ & $7.76$ & $7.76$ & $11.40$ & $8.76$ & $7.76$ \\ 
$10$ & $38$ & $9.95$ & $7.89$ & $7.89$ & $11.52$ & $8.76$ & $7.89$ \\ 
$10$ & $110$ & $11.19$ & $8.51$ & $8.51$ & $12.63$ & $11.26$ & $11.26$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_tablemean.tex <==
$2$ & $6$ & $4.31$ & $4.26$ & $3.93$ & $6.01$ \\ 
$2$ & $14$ & $5.42$ & $4.36$ & $4.17$ & $6.94$ \\ 
$4$ & $14$ & $5.21$ & $4.39$ & $4.19$ & $7.01$ \\ 
$4$ & $38$ & $6.72$ & $4.52$ & $4.53$ & $8$ \\ 
$10$ & $38$ & $6.62$ & $4.55$ & $4.53$ & $8.16$ \\ 
$10$ & $110$ & $7.63$ & $4.95$ & $4.95$ & $9.08$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_tablemean_asandkms.tex <==
$4.93$ & $4.74$ \\ 
$ $ & $ $ \\ 
$ $ & $ $ \\ 
$ $ & $ $\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_tablemean_coxandshi.tex <==
$2$ & $6$ & $4.31$ & $4.26$ & $3.93$ & $6.01$ & $5.04$ & $4.27$ \\ 
$2$ & $14$ & $5.42$ & $4.36$ & $4.17$ & $6.94$ & $5.16$ & $4.37$ \\ 
$4$ & $14$ & $5.21$ & $4.39$ & $4.19$ & $7.01$ & $5.21$ & $4.39$ \\ 
$4$ & $38$ & $6.72$ & $4.52$ & $4.53$ & $8$ & $5.35$ & $4.52$ \\ 
$10$ & $38$ & $6.62$ & $4.55$ & $4.53$ & $8.16$ & $5.39$ & $4.55$ \\ 
$10$ & $110$ & $7.63$ & $4.95$ & $4.95$ & $9.08$ & $7.30$ & $7.06$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_tablemean_zerocutoff.tex <==
$2$ & $6$ & $4.39$ & $4.35$ & $4.02$ & $6.09$ \\ 
$2$ & $14$ & $5.50$ & $4.45$ & $4.25$ & $7.02$ \\ 
$4$ & $14$ & $5.29$ & $4.48$ & $4.27$ & $7.10$ \\ 
$4$ & $38$ & $6.81$ & $4.60$ & $4.61$ & $8.09$ \\ 
$10$ & $38$ & $6.71$ & $4.64$ & $4.61$ & $8.24$ \\ 
$10$ & $110$ & $7.71$ & $5.03$ & $5.03$ & $9.16$\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_tablemean_zerocutoff_asandkms.tex <==
$5.02$ & $4.83$ \\ 
$ $ & $ $ \\ 
$ $ & $ $ \\ 
$ $ & $ $\\

==> Tables/Theta_g_Rejection_Probabilities_excess_length_tablemean_zerocutoff_coxandshi.tex <==
$2$ & $6$ & $4.39$ & $4.35$ & $4.02$ & $6.09$ & $5.13$ & $4.35$ \\ 
$2$ & $14$ & $5.50$ & $4.45$ & $4.25$ & $7.02$ & $5.25$ & $4.45$ \\ 
$4$ & $14$ & $5.29$ & $4.48$ & $4.27$ & $7.10$ & $5.29$ & $4.48$ \\ 
$4$ & $38$ & $6.81$ & $4.60$ & $4.61$ & $8.09$ & $5.43$ & $4.60$ \\ 
$10$ & $38$ & $6.71$ & $4.64$ & $4.61$ & $8.24$ & $5.48$ & $4.64$ \\ 
$10$ & $110$ & $7.71$ & $5.03$ & $5.03$ & $9.16$ & $7.38$ & $7.14$\\

==> Tables/Theta_g_Rejection_Probabilities_lower_bound_sizes.tex <==
$2$ & $6$ & $0.03$ & $0.03$ & $0.05$ & $0.00$ \\ 
$2$ & $14$ & $0.01$ & $0.03$ & $0.04$ & $0.00$ \\ 
$4$ & $14$ & $0.01$ & $0.03$ & $0.03$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.01$ & $0.01$ & $0.00$\\

==> Tables/Theta_g_Rejection_Probabilities_lower_bound_sizes_zerocutoff.tex <==
$2$ & $6$ & $0.03$ & $0.03$ & $0.04$ & $0.00$ \\ 
$2$ & $14$ & $0.01$ & $0.03$ & $0.04$ & $0.00$ \\ 
$4$ & $14$ & $0.01$ & $0.03$ & $0.03$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.02$ & $0.02$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.01$ & $0.01$ & $0.00$\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set.tex <==
$0.04$ & $0.04$ & $0.06$ & $0.01$ \\ 
$0.02$ & $0.05$ & $0.05$ & $0.00$ \\ 
$0.03$ & $0.04$ & $0.05$ & $0.00$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ \\ 
$0.00$ & $0.03$ & $0.03$ & $0.00$\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_allcombined_modified.tex <==
$0.04$ & $0.04$ & $0.06$ & $0.01$ & $0.02$ & $0.04$ & $0.03$ & $0.03$ \\ 
$0.02$ & $0.05$ & $0.05$ & $0.00$ & $0.03$ & $0.05$ & $0.02$ & $0.02$ \\ 
$0.03$ & $0.04$ & $0.05$ & $0.00$ & $0.03$ & $0.04$ & $0.02$ & $0.05$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.03$ & $0.05$ & $0.02$ & $0.08$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.03$ & $0.05$ & $ $ & $ $ \\ 
$0.00$ & $0.03$ & $0.03$ & $0.00$ & $0.02$ & $0.02$ & $ $ & $ $\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_asandkms.tex <==
$0.04$ & $0.04$ & $0.06$ & $0.01$ & $0.03$ & $0.03$ \\ 
$0.02$ & $0.05$ & $0.05$ & $0.00$ & $0.02$ & $0.02$ \\ 
$0.03$ & $0.04$ & $0.05$ & $0.00$ & $0.04$ & $0.05$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.07$ & $0.08$\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_coxandshi.tex <==
$0.04$ & $0.04$ & $0.06$ & $0.01$ & $0.02$ & $0.04$ \\ 
$0.02$ & $0.05$ & $0.05$ & $0.00$ & $0.03$ & $0.05$ \\ 
$0.03$ & $0.04$ & $0.05$ & $0.00$ & $0.03$ & $0.04$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.03$ & $0.05$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.03$ & $0.05$ \\ 
$0.00$ & $0.03$ & $0.03$ & $0.00$ & $0.02$ & $0.02$\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_zerocutoff.tex <==
$0.03$ & $0.04$ & $0.06$ & $0.01$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ \\ 
$0.00$ & $0.03$ & $0.03$ & $0.00$\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_zerocutoff_allcombined.tex <==
$0.03$ & $0.04$ & $0.06$ & $0.01$ & $0.02$ & $0.04$ & $0.02$ & $0.03$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ & $0.02$ & $0.04$ & $0.02$ & $0.02$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ & $0.02$ & $0.04$ & $0.04$ & $0.05$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ & $0.03$ & $0.04$ & $0.07$ & $0.08$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.02$ & $0.05$ & $ $ & $ $ \\ 
$0.00$ & $0.03$ & $0.03$ & $0.00$ & $0.02$ & $0.02$ & $ $ & $ $\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_zerocutoff_asandkms.tex <==
$0.03$ & $0.04$ & $0.06$ & $0.01$ & $0.02$ & $0.03$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ & $0.02$ & $0.02$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ & $0.04$ & $0.05$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ & $0.07$ & $0.08$\\

==> Tables/Theta_g_Rejection_Probabilities_max_size_in_id_set_zerocutoff_coxandshi.tex <==
$0.03$ & $0.04$ & $0.06$ & $0.01$ & $0.02$ & $0.04$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ & $0.02$ & $0.04$ \\ 
$0.02$ & $0.04$ & $0.05$ & $0.00$ & $0.02$ & $0.04$ \\ 
$0.00$ & $0.04$ & $0.04$ & $0.00$ & $0.03$ & $0.04$ \\ 
$0.00$ & $0.05$ & $0.05$ & $0.00$ & $0.02$ & $0.05$ \\ 
$0.00$ & $0.03$ & $0.03$ & $0.00$ & $0.02$ & $0.02$\\

==> Tables/Theta_g_Rejection_Probabilities_power_table05.tex <==
$2$ & $6$ & $-81.40$ & $-81.60$ & $-81.57$ & $-81.45$ & $-82.50$ & $38.65$ & $38.74$ & $38.70$ & $38.55$ & $39.58$ \\ 
$2$ & $14$ & $-81.40$ & $-82.29$ & $-81.76$ & $-81.58$ & $-83.04$ & $38.65$ & $39.16$ & $38.65$ & $38.57$ & $39.88$ \\ 
$4$ & $14$ & $-81.42$ & $-82.13$ & $-81.72$ & $-81.61$ & $-83.11$ & $38.66$ & $39.10$ & $38.73$ & $38.63$ & $39.95$ \\ 
$4$ & $38$ & $-81.42$ & $-83$ & $-81.82$ & $-81.82$ & $-83.69$ & $38.66$ & $39.65$ & $38.67$ & $38.68$ & $40.20$ \\ 
$10$ & $38$ & $-81.42$ & $-82.91$ & $-81.81$ & $-81.81$ & $-83.67$ & $38.66$ & $39.61$ & $38.69$ & $38.69$ & $40.33$ \\ 
$10$ & $110$ & $-81.42$ & $-83.52$ & $-82.05$ & $-82.05$ & $-84.25$ & $38.66$ & $39.97$ & $38.96$ & $38.95$ & $40.59$\\

==> Tables/Theta_g_Rejection_Probabilities_power_table50.tex <==
$2$ & $6$ & $-81.40$ & $-83.62$ & $-83.59$ & $-83.44$ & $-84.48$ & $38.65$ & $40.72$ & $40.68$ & $40.52$ & $41.54$ \\ 
$2$ & $14$ & $-81.40$ & $-84.27$ & $-83.72$ & $-83.61$ & $-85.09$ & $38.65$ & $41.17$ & $40.67$ & $40.60$ & $41.88$ \\ 
$4$ & $14$ & $-81.42$ & $-84.19$ & $-83.76$ & $-83.64$ & $-85.13$ & $38.66$ & $41.10$ & $40.71$ & $40.62$ & $41.97$ \\ 
$4$ & $38$ & $-81.42$ & $-85.07$ & $-83.85$ & $-83.86$ & $-85.78$ & $38.66$ & $41.73$ & $40.70$ & $40.70$ & $42.31$ \\ 
$10$ & $38$ & $-81.42$ & $-85.03$ & $-83.91$ & $-83.88$ & $-85.87$ & $38.66$ & $41.69$ & $40.72$ & $40.71$ & $42.41$ \\ 
$10$ & $110$ & $-81.42$ & $-85.69$ & $-84.34$ & $-84.34$ & $-86.50$ & $38.66$ & $42.08$ & $40.98$ & $40.99$ & $42.69$\\

==> Tables/Theta_g_Rejection_Probabilities_power_table95.tex <==
$2$ & $6$ & $-81.40$ & $-85.61$ & $-85.58$ & $-85.42$ & $-86.48$ & $38.65$ & $42.80$ & $42.78$ & $42.57$ & $43.58$ \\ 
$2$ & $14$ & $-81.40$ & $-86.29$ & $-85.69$ & $-85.62$ & $-87.07$ & $38.65$ & $43.17$ & $42.69$ & $42.62$ & $43.91$ \\ 
$4$ & $14$ & $-81.42$ & $-86.19$ & $-85.73$ & $-85.62$ & $-87.16$ & $38.66$ & $43.15$ & $42.79$ & $42.68$ & $44.04$ \\ 
$4$ & $38$ & $-81.42$ & $-87.08$ & $-85.86$ & $-85.88$ & $-87.75$ & $38.66$ & $43.80$ & $42.79$ & $42.80$ & $44.41$ \\ 
$10$ & $38$ & $-81.42$ & $-87$ & $-85.89$ & $-85.89$ & $-87.89$ & $38.66$ & $43.83$ & $42.83$ & $42.82$ & $44.48$ \\ 
$10$ & $110$ & $-81.42$ & $-87.73$ & $-86.43$ & $-86.35$ & $-88.61$ & $38.66$ & $44.18$ & $43.15$ & $43.13$ & $44.84$\\

==> Tables/Theta_g_Rejection_Probabilities_upper_bound_sizes.tex <==
$2$ & $6$ & $0.04$ & $0.04$ & $0.06$ & $0.01$ \\ 
$2$ & $14$ & $0.02$ & $0.05$ & $0.05$ & $0.00$ \\ 
$4$ & $14$ & $0.03$ & $0.04$ & $0.05$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.05$ & $0.05$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.05$ & $0.05$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.03$ & $0.03$ & $0.00$\\

==> Tables/Theta_g_Rejection_Probabilities_upper_bound_sizes_zerocutoff.tex <==
$2$ & $6$ & $0.03$ & $0.04$ & $0.06$ & $0.01$ \\ 
$2$ & $14$ & $0.02$ & $0.04$ & $0.05$ & $0.00$ \\ 
$4$ & $14$ & $0.02$ & $0.04$ & $0.05$ & $0.00$ \\ 
$4$ & $38$ & $0.00$ & $0.04$ & $0.04$ & $0.00$ \\ 
$10$ & $38$ & $0.00$ & $0.05$ & $0.05$ & $0.00$ \\ 
$10$ & $110$ & $0.00$ & $0.03$ & $0.03$ & $0.00$\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda05.tex <==
3 & 6 & 10.10 & 6.31 & 6.31 & 15.15 \\ 
3 & 14 & 0.25 & 0.15 & 0.10 & 0.35 \\ 
5 & 14 & 2.30 & 1.06 & 1.06 & 3.54 \\ 
5 & 38 & 0.35 & 0.25 & 0.05 & 0.50 \\ 
11 & 38 & 0.50 & 0.20 & 0.20 & 0.81 \\ 
11 & 110 & 0.35 & 0.66 & 0.05 & 0.55\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda05_coxandshi.tex <==
8.84 & 6.31 \\ 
0.15 & 0.10 \\ 
1.41 & 1.06 \\ 
0.10 & 0.05 \\ 
0.20 & 0.20 \\ 
0.15 & 0.15\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda05_zerocutoff.tex <==
3 & 6 & 10.10 & 6.31 & 6.31 & 15.15 \\ 
3 & 14 & 0.25 & 0.15 & 0.10 & 0.35 \\ 
5 & 14 & 2.65 & 1.41 & 1.41 & 3.89 \\ 
5 & 38 & 0.35 & 0.25 & 0.05 & 0.50 \\ 
11 & 38 & 0.50 & 0.20 & 0.20 & 0.81 \\ 
11 & 110 & 0.35 & 0.66 & 0.05 & 0.55\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda05_zerocutoff_coxandshi.tex <==
8.84 & 6.31 \\ 
0.15 & 0.10 \\ 
1.77 & 1.41 \\ 
0.10 & 0.05 \\ 
0.20 & 0.20 \\ 
0.15 & 0.15\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda50_zerocutoff.tex <==
3 & 6 & 61.87 & 42.93 & 36.62 & 118.69 \\ 
3 & 14 & 0.55 & 0.45 & 0.35 & 0.76 \\ 
5 & 14 & 8.13 & 6.36 & 5.66 & 10.61 \\ 
5 & 38 & 0.66 & 0.96 & 0.45 & 0.86 \\ 
11 & 38 & 1.01 & 1.01 & 0.81 & 1.41 \\ 
11 & 110 & 0.66 & 2.57 & 0.55 & 0.86\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda50_zerocutoff_coxandshi.tex <==
60.61 & 42.93 \\ 
0.45 & 0.35 \\ 
6.72 & 6.01 \\ 
0.40 & 0.35 \\ 
0.71 & 0.71 \\ 
0.45 & 0.45\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda95.tex <==
3 & 6 & 123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} \\ 
3 & 14 & 0.96 & 0.96 & 0.86 & 1.16 \\ 
5 & 14 & 31.29\rlap{$^{+}$} & 31.29\rlap{$^{+}$} & 27.58 & 31.29\rlap{$^{+}$} \\ 
5 & 38 & 0.96 & 4.21\rlap{$^{+}$} & 0.96 & 1.16 \\ 
11 & 38 & 1.92 & 7.01\rlap{$^{+}$} & 1.72 & 2.42 \\ 
11 & 110 & 0.96 & 5.70\rlap{$^{+}$} & 0.91 & 1.26\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda95_coxandshi.tex <==
123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} \\ 
0.86 & 0.83 \\ 
31.29\rlap{$^{+}$} & 28.11 \\ 
0.76 & 0.76 \\ 
1.51 & 1.51 \\ 
0.86 & 0.86\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda95_zerocutoff.tex <==
3 & 6 & 123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} \\ 
3 & 14 & 0.96 & 0.96 & 0.86 & 1.16 \\ 
5 & 14 & 31.64\rlap{$^{+}$} & 31.64\rlap{$^{+}$} & 27.93 & 31.64\rlap{$^{+}$} \\ 
5 & 38 & 0.96 & 4.21\rlap{$^{+}$} & 0.96 & 1.16 \\ 
11 & 38 & 1.92 & 7.01\rlap{$^{+}$} & 1.72 & 2.42 \\ 
11 & 110 & 0.96 & 5.70\rlap{$^{+}$} & 0.91 & 1.26\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambda95_zerocutoff_coxandshi.tex <==
123.11\rlap{$^{+}$} & 123.11\rlap{$^{+}$} \\ 
0.86 & 0.83 \\ 
31.64\rlap{$^{+}$} & 28.46 \\ 
0.76 & 0.76 \\ 
1.51 & 1.51 \\ 
0.86 & 0.86\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambdamean.tex <==
3 & 6 & 69.83\rlap{$^{+}$} & 60.10\rlap{$^{+}$} & 56.03\rlap{$^{+}$} & 84.17\rlap{$^{+}$} \\ 
3 & 14 & 0.58 & 0.49\rlap{$^{+}$} & 0.42 & 0.74 \\ 
5 & 14 & 10.45\rlap{$^{+}$} & 10.41\rlap{$^{+}$} & 7.93\rlap{$^{+}$} & 13.51\rlap{$^{+}$} \\ 
5 & 38 & 0.64 & 1.34\rlap{$^{+}$} & 0.48 & 0.85 \\ 
11 & 38 & 1.08 & 2.02\rlap{$^{+}$} & 0.84 & 1.49 \\ 
11 & 110 & 0.65 & 2.80\rlap{$^{+}$} & 0.51 & 0.89\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambdamean_coxandshi.tex <==
69.09\rlap{$^{+}$} & 59.99\rlap{$^{+}$} \\ 
0.46\rlap{$^{+}$} & 0.41\rlap{$^{+}$} \\ 
9.10\rlap{$^{+}$} & 8.25\rlap{$^{+}$} \\ 
0.43 & 0.41 \\ 
0.76 & 0.73 \\ 
0.45 & 0.45\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambdamean_zerocutoff.tex <==
3 & 6 & 69.83\rlap{$^{+}$} & 60.10\rlap{$^{+}$} & 56.03\rlap{$^{+}$} & 84.17\rlap{$^{+}$} \\ 
3 & 14 & 0.58 & 0.49\rlap{$^{+}$} & 0.42 & 0.74 \\ 
5 & 14 & 10.81\rlap{$^{+}$} & 10.76\rlap{$^{+}$} & 8.28\rlap{$^{+}$} & 13.86\rlap{$^{+}$} \\ 
5 & 38 & 0.64 & 1.34\rlap{$^{+}$} & 0.48 & 0.85 \\ 
11 & 38 & 1.08 & 2.02\rlap{$^{+}$} & 0.84 & 1.49 \\ 
11 & 110 & 0.65 & 2.80\rlap{$^{+}$} & 0.51 & 0.89\\

==> Tables/lambda_rejection_probabilities_excess_length_table_lambdamean_zerocutoff_coxandshi.tex <==
69.09\rlap{$^{+}$} & 59.99\rlap{$^{+}$} \\ 
0.46\rlap{$^{+}$} & 0.41\rlap{$^{+}$} \\ 
9.45\rlap{$^{+}$} & 8.60\rlap{$^{+}$} \\ 
0.43 & 0.41 \\ 
0.76 & 0.73 \\ 
0.45 & 0.45\\

==> Tables/lambda_rejection_probabilities_max_size_in_id_set_zerocutoff.tex <==
\\

==> Tables/lambda_rejection_probabilities_max_size_in_id_set_zerocutoff_coxandshi.tex <==
$0.00$ & $0.00$ \\ 
$0.00$ & $0.01$ \\ 
$0.00$ & $0.01$ \\ 
$0.02$ & $0.02$ \\ 
$0.00$ & $0.01$ \\ 
$0.01$ & $0.01$\\

==> Tables/lambda_rejection_probabilities_upper_bound_sizes_lambda.tex <==
$3$ & $6$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\ 
$3$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$5$ & $14$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$5$ & $38$ & $0.00$ & $0.03$ & $0.02$ & $0.00$ \\ 
$11$ & $38$ & $0.00$ & $0.01$ & $0.01$ & $0.00$ \\ 
$11$ & $110$ & $0.00$ & $0.05$ & $0.04$ & $0.00$\\

==> Tables/lambda_rejection_probabilities_upper_bound_sizes_lambda_zerocutoff.tex <==
$3$ & $6$ \\ 
$3$ & $14$ \\ 
$5$ & $14$ \\ 
$5$ & $38$ \\ 
$11$ & $38$ \\ 
$11$ & $110$\\
